Sublinear-Time Sampling of Spanning Trees in the Congested Clique

We present the first sublinear-in-$n$ round algorithm for sampling an approximately uniform spanning tree of an $n$-vertex graph in the CongestedClique model of distributed computing. In particular, our algorithm requires $\Tilde{O}(n^{0.657})$ rounds for sampling a spanning tree within total variation distance $1/n^c$, for arbitrary constant $c > 0$, from the uniform distribution. More precisely, our algorithm requires $\Tilde{O}(n^{1/2 + \alpha})$ rounds, where $O(n^\alpha)$ is the running time of matrix multiplication in the CongestedClique model (currently $\alpha = 1 - 2/\omega = 0.157$, where $\omega$ is the sequential matrix multiplication time exponent). We can adapt our algorithm to give exact rather than approximate samples, but with a larger, though still $o(n)$, runtime of $\Tilde{O}(n^{2/3+\alpha}) = O(n^{.824})$. In a remarkable result, Aldous (SIDM 1990) and Broder (FOCS 1989) showed that the first visit edge to each vertex, excluding the start vertex, during a random walk forms a uniformly chosen spanning tree of the underlying graph. Our algorithm is a significant departure from known techniques, featuring a top-down walk filling approach paired with Schur complement graphs for walk shortcutting. To make this idea work in the CongestedClique model, we present a novel compressed random walk reconstruction algorithm, based on randomly sampling a weighted perfect matching. In addition, we show how to take somewhat shorter random walks even more efficiently in the CongestedClique model, obtaining an $O(\log^3 n)$-round algorithm for uniformly sampling spanning trees from graphs with $O(n\log n)$ cover times. These results are obtained by adding a load balancing component to the random walk algorithm of Bahmani, Chakrabarti and Xin (SIGMOD 2011) that uses the bottom-up ``doubling'' technique.

==> FastWalk.tex <==
\section{Warm-up: Fast Random Walks via Doubling}\label{section:fastWalk}
Bahmani, Chakrabarti, and Xin \cite{BCX} present an algorithm called \dbling that computes a random walk of length $\lambda$ in $O(\log \lambda)$ iterations in the Map-Reduce model. 
A single iteration in the Map-Reduce model may require $\Omega(n)$ rounds in the \cc{} model and so using the \dbling directly in the \cc{} model is not efficient. 
In this section we present a ``load balanced'' version of the \dbling algorithm that can compute a length-$n$ walk in $\pln$ rounds in the \cc{} model.

\smallskip

\noindent
\textbf{High-level idea.} To compute a length-$n$ random walk, the \dbling algorithm starts with each vertex $v$ computing $n$ length-1 walks originating at $v$. At each iteration, walks ending at a node $v$ are merged with walks originating at $v$. This halves the number of walks held by a vertex, while doubling the length of every walk. After $O(\log n)$ of these ``doubling'' iterations, every node $v$ holds a length-$n$ random walk originating at vertex $v$. While each walk is a proper random walk, 
because of how the walks are merged, walks originating at different vertices are not independent.  
The main challenge for the \dbling algorithm is to implement the merging step efficiently in the \cc{} model. 
Specifically, a faithful implementation of the \dbling algorithm may require $\Omega(n^2 \log n)$ bits to travel to a particular vertex in a single merging step, which 
requires $\Omega(n)$ rounds in the \cc{} model. 
We add a ``load balancing'' step to each merging step so as to take advantage of the 
overall $\Theta(n^2)$ bandwidth of the \cc{} model.
We show that with this ``load balancing'' step in place, each merging step takes $O(\log n)$ rounds, w.h.p.

\smallskip

\noindent
\textbf{Load-balanced Doubling Algorithm.} We now describe our algorithm.
Consider an iteration of the \dbling algorithm. We assume that just before the start of this iteration, each vertex holds a sequence of $k$ walks of length $\ell$ each. 
Let $W_v^1, W_v^2, \ldots, W_v^k$ denote the sequence of $k$ length-$\ell$ walks held by vertex $v$.
We further assume that both $k$ and $\ell$ are powers of 2 and $k \cdot \ell$ is the smallest power of 2 that is at least $n$. Before the first iteration, $k$ is the smallest power of 2 that is at least 2 and $\ell$ is 1. After each iteration, $k$ halves and $\ell$ doubles.

\begin{enumerate}
\item A leader vertex (e.g., vertex with lowest \id) picks a binary string $s$ of length $O(n \log n)$ uniformly at random. The leader broadcasts $s$ to all vertices.
Every vertex then uses $s$ to pick a hash function $h_s$ from a family of $n$-wise independent hash functions $\mathcal{H} = \{h : \mathcal{I} \times [k] \to \mathcal{I}\}$. Here $\mathcal{I}$ is the set of \id's of the vertices.

\item For $i=1, 2, \dots, k/2:$ each vertex $v$ sends the tuple $(\id_v, i, W_v^i)$ to the vertex with \id $=h_s(\text{lastID}(W_v^i), k-i)$.

\item For $i=k/2+1,\dots, k:$ each vertex $v$ sends $(\id_v, i, W_v^i)$ to the vertex whose \id is $h_s(\id_v, i)$.

\item Each vertex $w$ receiving two walks $W_u^i$ and $W_v^j$, where $\text{lastID}(W_u^i) = \id_v$, $1 \le i \le k/2$, and $i + j = k$ concatenates $W_u^i$ and $W_v^j$ and sends the tuple $(i, W_u^i \circ W_v^j)$ to vertex $u$.

\item Each vertex $v$, on receiving a tuple $(i, W)$, sets $W_v^i := W$.
\end{enumerate}


